The Illusion of State in State-Space Models

State-space models (SSMs) have emerged as a potential alternative architecture for building large language models (LLMs) compared to the previously ubiquitous transformer architecture. One theoretical weakness of transformers is that they cannot express certain kinds of sequential computation and state tracking (Merrill & Sabharwal, 2023), which SSMs are explicitly designed to address via their close architectural similarity to recurrent neural networks (RNNs). But do SSMs truly have an advantage (over transformers) in expressive power for state tracking? Surprisingly, the answer is no. Our analysis reveals that the expressive power of SSMs is limited very similarly to transformers: SSMs cannot express computation outside the complexity class $\mathsf{TC}^0$. In particular, this means they cannot solve simple state-tracking problems like permutation composition. It follows that SSMs are provably unable to accurately track chess moves with certain notation, evaluate code, or track entities in a long narrative. To supplement our formal analysis, we report experiments showing that Mamba-style SSMs indeed struggle with state tracking. Thus, despite its recurrent formulation, the "state" in an SSM is an illusion: SSMs have similar expressiveness limitations to non-recurrent models like transformers, which may fundamentally limit their ability to solve real-world state-tracking problems.

==> old/camera-ready-refactor.tex <==
\will{===== OLD =====}

\begin{definition}[Linear SSM layer; e.g.~S4]
    \label{defn:linear-ssm-layer}
    Given a sequence of embeddings or previous states $x_1, \ldots, x_n \in \mathbb R^m$, the \emph{recurrent form} of a linear SSM layer defines a new sequence of states $h_1, \ldots, h_n \in \mathbb R^d$ using learned parameter matrices $A \in \mathbb R^{d \times d}$ and $B \in \mathbb R^{d \times m}$. For each $1 \leq i \leq n$,
    \begin{equation}
        \label{eqn:s4-recurrent}
        h_i = A h_{i-1} + B x_i .
    \end{equation}
    % where $\overline{A},\overline{B}$ are the discretizations of $A$ and $B$.
    The \emph{convolutional form} of the linear SSM layer defines the same\footnote{The two forms express the same function over $\mathbb R$ or any other distributive datatype. Over floating points (\Cref{sec:arithmetic}), they are not guaranteed to be the same, but we must assume the error is negligible for them to be well-defined and usable in practice.} $h_1, \ldots, h_n$ but is unrolled as a summation of terms:
    \begin{equation}
        \label{eqn:s4-convolutional}
        h_i = \sum_{j=1}^{i} A^{(i-j)} B x_j .
    \end{equation}
    The layer outputs $y_i = C h_i + D x_i$ where $C \in \mathbb R^{d \times m}$ and $D \in \mathbb R^{m \times m}$.
    % \begin{equation}
    %     \label{eqn:s4-output}
    %     y_i = C h_i + D x_i .
    % \end{equation}
\end{definition}

S4 chooses a specific parameterization of a linear layer.
A full S4 model is a cascade of such layers and feedforward layers, analogous to how transformers alternate multihead-self-attention layers with feedforward layers.

The S6 layer used by Mamba \citep{gu2023mamba} generalizes a linear SSM layer by adding a \emph{selection mechanism} inspired by the dynamic gating in LSTMs \citep{hochreiter1997long} and GRUs \citep{cho-etal-2014-learning}.

\begin{definition}[S6 layer] \label{def:s6-layer}
An S6 layer is parameterized by a \emph{diagonal} matrix $A \in \mathbb R^{d \times d}$, a vector $\delta \in \mathbb{R}^d$, and affine projections $s_\delta : \mathbb{R}^m \to \mathbb{R}^d, s_B : \mathbb{R}^m \to \mathbb{R}^d,$ and $s_C : \mathbb{R}^d \to \mathbb{R}^m$. 
Let $\tau$ be softplus.
The S6 layer is:
% S6 adds a scalar factor $\delta_i \in [0, 1]$ modulating how much the previous state is remembered as a function of $x_i$ and also allows $B$ to depend on $x_i$:
\begin{align}
    h_i &= \overline{A}_i h_{i-1} + \overline{B}_i x_i , \label{eqn:s6-recurrent} \\
    \textrm{where} \; \delta_i &= \tau(\delta + s_\delta(x)) \; \textrm{and} \notag \\
    \; B_i &= s_B(x), \notag
\end{align}
where 
$$\overline{A}_i \triangleq \exp(\delta_i A), \quad \overline{B}_i \triangleq (\delta_i A)^{-1}(\exp(A) - I) \cdot \delta_i B_i$$ are the discretizations of $A$ and $B$.
% S6 also adds the constraint \ashish{instead of this piecemeal description, can we add a concrete definition of an S6 layer, similar to \Cref{defn:linear-ssm-layer}, for which we will prove results?} that $A$ must be a \emph{diagonal} matrix.
This admits the convolutional form:
% (cf.~\Cref{sec:s6-conv-derivation}):
% \begin{equation} \label{eqn:s6-convolutional}
%     h_i = \sum_{j=1}^i \exp \left( A \sum_{k=j+1}^i  \delta_k \right) B_j x_j .
% \end{equation}
\begin{equation} \label{eqn:s6-convolutional}
    h_i = \sum_{j=1}^i \left( \prod_{k=j+1}^i \overline{A}_k \right) \overline{B}_j x_j .
\end{equation}
Finally, to compute $y_i$, $C$ is made input dependent $C_i$ and computed via a projection in the same manner as $B_i$. The layer output is then $y_i = C_i h_i + x_i$.
\end{definition}

\begin{remark}
    The use of discretized $\overline{A},\overline{B}$ for the recurrent and convolution forms in \cref{def:s6-layer} is needed to approximate the continuous dynamical system with fixed precision. This is true also in the case of and S4 layer, but in \cref{defn:linear-ssm-layer} we omit the discretized versions because the discretization step is not input-dependent. This means that the discretized $\overline{A},\overline{B}$ can be computed just once, and so without a loss of generality we can consider $A$ and $B$ to already be discretized. This is not the case for S6, where the input-dependence of the discretized forms means we must recompute $\overline{A},\overline{B}$ for each input.
\end{remark}

% \ashish{I think we should be mathematically more precise here. E.g., the use of $B_i$ suggests $B$ can be a function of $i$. But that will make the circuit simulation \textbf{non-uniform}, just because there can be an unbounded number of different $B$'s! What exactly do we mean here? If $x_i$ were only token embeddings, we could think of $B(x_i)$ instead as there would only be as many as $\abs{\Sigma}$ (vocabulary size) distinct ones. But even this doesn't quite work if $x_i$ are the outputs of the previous layer. Hmm... what do they assume in practice? $B_i$ with bounded $i$? Should we formally think of $B_i \in \mathbf{B}$ where the latter is some finite set?}

\will{===== Old subsections below here =====}

\subsection{Simulating Linear SSMs with a $\TC^0$ Circuit Family}

\begin{theorem} \label{thm:s4}
    For any log-precision SSM $M$ with the S4 architecture, there exists an $\L$-uniform $\TC^0$ circuit family that computes the same function as $M$'s convolutional form.
\end{theorem}

\begin{proof}
    It suffices to construct an $\L$-uniform $\TC^0$ circuit family to simulate a single layer. Then, the full SSM can be simulate by generating this circuit multiple times, routing the output bits from one layer as the inputs to the next. This can be done with log-space overhead by simply storing a counter that tracks the index of the current input gates.

    Recall that the S4 convolutional form Eqn.~\eqref{eqn:s4-convolutional} is $h_i = \sum_{j=1}^{i} A^{(i-j)} B x_j$. Crucially, we use the fact that matrix powering over floats is in $\L$-uniform $\TC^0$ (\Cref{cor:float-matrix-power}, extending \citealp{mereghetti2000threshold}) to print, for each $i, j$, a $\TC^0$ circuit family that computes $\pi_{ij} \triangleq A^{(i-j)}$.
    Next, we use the fact that fixed-arity arithmetic over floats is in $\L$-uniform $\TC^0$ to print, for each $i, j$, a circuit that computes
    \begin{equation*}
        \tau_{ij} \, \triangleq \, \pi_{ij} B x_j \, = \, A^{(i-j)} B x_j .
    \end{equation*}
    Since iterated addition over floats is in $\L$-uniform $\TC^0$ (\citealp{merrill-sabharwal-2023-parallelism}, extending \citealp{hesse2001division,Chiu2001DivisionIL} for integers), we can compute $h_i \triangleq \sum_{j=1}^i \tau_{ij}$.
    Finally, we compute $y_i$ from $x_i$ and $h_i$ in $\TC^0$ via simple arithmetic operations, completing the proof.
\end{proof}

\subsection{Simulating S6 with a $\TC^0$ Circuit Family}

\begin{theorem} \label{thm:s6}
    For any log-precision SSM $M$ with the S6 architecture, there exists an $\L$-uniform $\TC^0$ circuit family that computes the same function as $M$'s convolutional form.
\end{theorem}

\begin{proof}
    The convolutional form of the S6 layer is given in Eqn.~\eqref{eqn:s6-convolutional}.
    % \begin{equation*}
    %     h_i
    %     % = \sum_{j=1}^i \left( \prod_{k=j+1}^i \delta(x_k) A \right) Bx_j .
    %     = \sum_{j=1}^i \exp \left( A \sum_{k=j+1}^i  \delta_k \right) B_i x_i ,
    % \end{equation*}
    % where $A$ is diagonal.
    For each $i$ we print an $\L$-uniform $\TC^0$ circuit computing $\delta_i, B_i$ and $C_i$.
    Since $A$ is diagonal, iterated matrix multiplication is reducible to iterated scalar multiplication, which is in $\L$-uniform $\TC^0$ (\Cref{cor:float-matrix-power}).
    so we can compute the following in $\TC^0$:
    \begin{equation*}
        \pi_{ij} \triangleq \prod_{k=j+1}^i \exp(\delta_k A) .
    \end{equation*}
    We then conclude analogously to \Cref{thm:s4}, first computing $\tau_{ij}$ from $\pi_{ij}$ and $\overline{B}_i$, then computing $h_i = \sum_{j=1}^i \tau_{ij}$, and finally computing $y_i$ from $x_i, h_i,$ and $C_i$ in $\TC^0$.
    \jackson{We probably need to justify here why the discretization of $B_i$ is $\TC^0$-computable}
\end{proof}

% \begin{remark}
%     The condition of $A$ being diagonal comes from the definition and implementation of S6 in \citet{gu2023mamba}. However, we show in \cref{sec:s6-conv-derivation} that the result still holds when $A$ is merely \emph{diagonalizable} and full-rank.
% \end{remark}

==> old/float-product.tex <==
\begin{definition}[Iterated $\D$-product]
    \label{defn:iterated-D-product}
    For $\phi_1, \ldots, \phi_z \in \D$, their \emph{iterated $\D$-product} is:
    \begin{equation}
        \bigotimes_{i=1}^z \phi_i \, \triangleq \, \cast_\D \left( \prod_{i=1}^z \cast_\R( \phi_i ) \right) .
    \end{equation}
\end{definition}
Here $\cast_\R$ converts a number in $\D$ to the corresponding real number. $\D$ is implicit in the notations $\cast_\R$ and $\bigotimes$.

\begin{lemma}[Iterated $\D$-product]
    \label{lem:iterated-D-product}
    Let $\phi_1, \ldots, \phi_z \in \D$ be such that $z \leq n$ and each $\phi_i$ can be represented as an $n$-bit integer. If operators $\cast_\D$ and $\cast_\R$ are in $\L$-uniform $\TC^0$, then the iterated $\D$-product $\bigotimes_{i=1}^z \phi_i$ can be computed in $\L$-uniform $\TC^0$.
\end{lemma}

\begin{proof}
    By preconditions of the lemma, we can compute $y_i = \cast_\R( \phi_i )$ for each $i$ in $\L$-uniform $\TC^0$. Since each $\phi_i$ is equivalent to an $n$-bit integer, $y_i$ can be viewed as an $n$-bit integer. The iterated integer product $y = \prod_{i=1}^z y_i$ can be computed with an $\L$-uniform $\TC^0$ circuit \cite{hesse2001division}. Finally, by a precondition of the lemma, we can cast the result back to $\D$, i.e., compute $\cast_\D ( y )$ which equals the iterated $\D$-product $\bigotimes_{i=1}^z \phi_i$, with an $\L$-uniform $\TC^0$ circuit.
\end{proof}

\floatproduct*

\begin{proof}
    The idea is to convert (by scaling up) the sequence of $\phi_i$ to another sequence of floats that are all representable as integers, apply \cref{lem:iterated-D-product}, reverse the scaling, and cast the result back to a $c \log n$ precision float.

    Let $e$ be the smallest exponent across all $\phi_i$ and $q = \max \{0, -e\}$. Construct re-scaled floats $\psi_i = \phi_i 2^q$ by adding $q$ to the exponent of $\phi_i$, using up to $c \log n$ additional bits in the exponent if necessary to keep the computation exact. Note that $e$, $q$, and all $\psi_i$ can easily be computed exactly by an $\L$-uniform $\TC^0$ circuit as they involve fixed-arity arithmetic operations. Further, by construction, every $\psi_i$ has a non-negative exponent and thus represents an integer.
    
    % Let $m = c \log n + n^c + 2^q$. Note that $2^q \in [0, n^c]$: hence, $m \leq c \log n + 2n^c$.
    The maximum number representable by each $c \log n$ precision float $\phi_i$ is upper bounded by $2^{n^c}$. Thus, the maximum number representable by each entry $\psi_i$ is $2^{n^c} \times 2^q = 2^{n^c + q}$. Let $m = n^c + q$. It follows that each $\psi_i$ can be equivalently represented as an $m$-bit integer. Further, this integer can be computed by left-shifting the mantissa of $\psi_i$ by a number of bits equal to the value of the exponent of $\psi_i$ (which is non-negative). Finally, this left-shift, and thus the $\cast_\R$ operation over $m$-precision floats, can be easily computed by an $\L$-uniform threshold circuit of size $\poly(m)$. In the other direction, casting from reals to $m$-precision floats can also be easily accomplished by an $\L$-uniform threshold circuit of size $\poly(m)$.

    Observing that $\psi_1, \ldots, \psi_z$ is a sequence of
    % $m$-bit floats,
    floats each representable as an $m$-bit integer,
    we now apply \cref{lem:iterated-D-product} with $\D$ being `float' to conclude that iterated float product $\tau = \bigotimes_{i=1}^z \psi_i$ can be computed by an $\L$-uniform threshold circuit of size $\poly(m)$. Since
    % $m \leq c \log n + 2n^c$,
    $m \leq 2n^c$,
    this circuit is also of size $\poly(n)$.

    Finally, to compute the original iterated float product $\bigotimes_{i=1}^z \phi_i$, we divide $\tau$ by $2^{qz}$. This can be accomplished by subtracting $qz$ from the exponent of $\tau$; again, we do this computation exactly, using up to $(c+1) \log n$ additional bits in the exponent if necessary. We then cast the resulting float back to a $c \log n$ precision float. All this can be done in $\L$-uniform $\TC^0$, finishing the proof that $\bigotimes_{i=1}^z \phi_i$ can be computed in $\L$-uniform $\TC^0$.
\end{proof}

We now extend these notions and results to matrix powering.

==> old/for-camera-ready.tex <==
%%%%%%%%%%%%%%%%%%%%
% TODOs for camera-ready:
% 1. General statement for different SSM variants
% 2. Move datatype details to appendix
% 3. Minimize technical jargon in intro?
% 4. Experiments: add appendix with length generalization id-s4
% 5. Emphasize importance of notation

%%%%%%%%%%%%%%%%%%%%
% GENERAL STATEMENT
%%%%%%%%%%%%%%%%%%%%

\ashish{How about stating our results for the following two settings? The motivation being to state the strongest result we know how to prove, and then point out how some existing architectures are special cases of it. On that note, are there any other specific architectures out there which might be special cases, besides just S4 and S6?
\begin{itemize}
    \item Generalized linear SSM layer: $h_i = \delta_i A h_{i-1} + B_i x_i$, where S4 is a special case with $\delta_i = 1$ and $B_i = B$
    \item Generalized exponential SSN layer: $h_i = \exp(\delta_i A) h_{i-1} + B_i x_i$ for some \emph{diagonalizable} $A$, where S6 is a special case with $A$ being diagonal
\end{itemize}
Ideally, I would like to generalize the latter of these to a broader non-linear case. Is there a candidate non-linear function (besides $\exp$) that might be easy to include?
}

==========================\\

\ashish{here is one attempt at what's on my mind:}
\will{Hmm, this seems to sacrifice a lot of readability for not much gain in generality.}

\begin{definition}[Generalized SSM, Recurrent Form]
    \label{defn:generalized-ssm-recurrent}
    A generalized State Space Model (SSM) $M$ is defined by a hidden dimension $d \in \Z^+$, a datatype $\D$, and a cascade of $L \geq 1$ SSM layers alternating with feedforward layers. On input $x^0_1, \ldots, x^0_n \in \D^d$, the output of $M$ is $x^L_1, \ldots, x^L_n \in \D^d$, computed as follows.
    For $\ell \geq 1$, let $x^{\ell-1}_1, \ldots, x^{\ell-1}_n \in \D^d$ denote the input to SSM layer $\ell$, and let $y^\ell_1, \ldots, y^\ell_n \in \D^d$ denote its output. For $\ell \geq 1$, the $\ell$-th feedforward (FFN) layer of $M$ maps each $y^\ell_i$ to $x^\ell_i$. In the $\ell$-th SSM layer of $M$, the \emph{hidden state computation} takes one of the following forms:
    \begin{align}
        \text{Linear:} && h^\ell_i & = \delta^\ell_i A^\ell h^\ell_{i-1} + B^\ell_i x^{\ell-1}_i \\
        \text{Polynomial:} && h^\ell_i & = \left(\delta^\ell_i A^\ell\right)^{k^\ell_i} h^\ell_{i-1} + B^\ell_i x^{\ell-1}_i \\
        \text{Exponential:} && h^\ell_i & = \exp\left(\delta^\ell_i A^\ell\right) h^\ell_{i-1} + B^\ell_i x^{\ell-1}_i
    \end{align}
    where $h^\ell_i \in \D^d$ and $\delta^\ell_i \in \D$, $k^\ell_i \in \Z^+$, and $A^\ell, B^\ell_i \in \D^{d \times d}$ are parameters of $M$. 
    Similarly, in the $\ell$-th SSM layer of $M$, the \emph{output computation} takes one of the following forms:
    \begin{align}
        \text{Linear:} && y^\ell_i & = \bar{\delta}^\ell_i C^\ell h^\ell_i + D^\ell_i x^{\ell-1}_i \\
        \text{Polynomial:} && y^\ell_i & = \left(\bar{\delta}^\ell_i C^\ell\right)^{\bar{k}^\ell_i} h^\ell_i + D^\ell_i x^{\ell-1}_i \\
        \text{Exponential:} && y^\ell_i & = \exp\left(\bar{\delta}^\ell_i C^\ell\right) h^\ell_i + D^\ell_i x^{\ell-1}_i
    \end{align}
    where $\bar{\delta}^\ell_i \in \D$, $\bar{k}^\ell_i \in \Z^+$, and $C^\ell, D^\ell_i \in \D^{d \times d}$ are parameters of $M$.
    We assume that parameters $\delta^\ell_i, \bar{\delta}^\ell_i, k^\ell_i, \bar{k}^\ell_i, B^\ell_i,$ and $D^\ell_i$ are functions only of $\ell$ and $x^0_i$,\footnote{More generally, our results hold as long as there is an $\L$-uniform $\TC^0$ computable mapping from $\ell, i,$ and a bounded part of the input to these parameters, such as a mapping from $\ell, i,$ and $x_i$ into a fixed set of parameter vectors and matrices.} and that in the exponential form of the SSM layer, parameter matrices $A^\ell$ and $C^\ell$ are diagonalizable.
\end{definition}

\ashish{double-check above equations for accuracy}

Note that this generalized SSM formulation allows different forms of hidden state computation layers and output computation layers to be combined arbitrarily within in a single SSM.

\begin{proposition}
    The S4 model is a generalized SSM with linear hidden state and output computation layers, with $\delta^\ell_i = \bar{\delta}^\ell_i = 1, B^\ell_i = B,$ and $D_i = D$.
\end{proposition}

\begin{proposition}
    The S6 model is a generalized SSM with exponential hidden state computation layers and linear output computation layers, with $A^\ell$ being a diagonal matrix.
\end{proposition}

\begin{definition}[Generalized SSM, Convolutional Form]
    \label{defn:generalized-ssm-convolutional}
    The convolutional form of a generalized SSM $M$ is the same as its recurrent form (\Cref{defn:generalized-ssm-recurrent}) except the \emph{hidden state computation} takes one of the following non-recurrent linear, polynomial, or exponential forms:
    \begin{align}
        h^\ell_i & = \sum_{j=1}^{i} \left(\prod_{k=j+1}^i \delta^\ell_k\right) (A^\ell)^{i-j} B^\ell_j x^{\ell-1}_j \\
        h^\ell_i & = \sum_{j=1}^{i} \left(\prod_{k=j+1}^i (\delta^\ell_k)^{k^\ell_i}\right) (A^\ell)^{\sum_{k=j+1}^i k^\ell_i} B^\ell_j x^{\ell-1}_j \\
        h^\ell_i & = \sum_{j=1}^{i} \exp\left(A^\ell \sum_{k=j+1}^i \delta^\ell_k \right) B^\ell_j x^{\ell-1}_j
    \end{align}
\end{definition}


\ashish{double-check above equations for accuracy}

\ashish{we can very briefly summarize the Numeric Datatype section here (move details to the appendix), define log-precision, and state the following main theorem:}

\begin{theorem}
    For any log-precision generalized SSM $M$, there exists an $\L$-uniform $\TC^0$ circuit family that computes the same function as $M$'s convolutional form.
\end{theorem}

\will{Ashish asked how the diagonalizable argument goes through. The idea is to prove that \Cref{lem:diagonalizable-conv-form} can be computed in $\TC^0$.}

==========================

\section{Derivation of S6 Convolutional Form} \label{sec:s6-conv-derivation}

% \subsection{Sum Version of S6 Conv Form}
% \will{No longer needed?}

% Over real numbers, the S6 recurrent form admits an equivalent convolutional form.

% \begin{lemma}
%     Let $h_0 = \vec 0 \in \mathbb R^d$ and $h_i = \exp( \delta_i A ) h_{i-1} + B_i x_i \in \mathbb R^d$.
%     Let $A$ be diagonal.
%     Then for any $i \geq 0$,
%     \begin{equation*}
%         h_i = \sum_{j=1}^i \exp \left( A \sum_{k=j+1}^i  \delta_k \right) B_i x_i .
%     \end{equation*}
% \end{lemma}

% \begin{proof}
%     We leverage the key property that $A$ is diagonal to use $\exp$ identities for scalars:
%     \begin{align*}
%         h_i
%         &= \exp( \delta_i A ) h_{i-1} + B_i x_i  \\
%         &= \sum_{j=1}^i \left( \prod_{k=j+1}^i \exp( \delta_k A ) \right) B_i x_i \\
%         &= \sum_{j=1}^i \exp \left( A \sum_{k=j+1}^i  \delta_k \right) B_i x_i . \qedhere
%     \end{align*}
% \end{proof}

\subsection{Extention to Full-Rank Diagonalizable $A$}

In S6, the transition matrix $A$ is diagonal, which very directly shows it can be simulated in $\TC^0$. We can strengthen this result to cover all cases when $A$ is \emph{diagonalizable} and full-rank.

\begin{lemma} \label{lem:factor_exp}
    Let $A$ be diagonalizable as $WDW^{-1}$. Then $\exp(A) = W \exp(D) W^{-1}$.
\end{lemma}
% \begin{proof}
%     \begin{align*}
%         \exp(A) &= \exp(WDW^{-1}) \tag{diagonalizable} \\
%         &= \sum_{k=0}^\infty \frac{1}{k!} (WDW^{-1})^k \tag{def. of $\exp$} \\
%         &= \sum_{k=0}^\infty \frac{1}{k!}WD^kW^{-1} \tag{cancellation} \\
%         &= W(\sum_{k=0}^\infty \frac{1}{k!}D^k)W^{-1} \tag{$\times$ associative} \\
%         &= W\exp(D)W^{-1} \tag*{\qedhere}
%     \end{align*}
% \end{proof}

\begin{lemma} \label{lem:factor_log}
    Let $A$ be full-rank and diagonalizable as $WDW^{-1}$. Then $\log A = W \log(D) W^{-1}$.
\end{lemma}

\begin{remark}
    We require $A$ to be full-rank to ensure that $\log A$ exists.
\end{remark}

% \begin{remark}
%     In general, the logarithm of a real matrix exists whenever it is invertible. However, there is no guarantee that $\log A$ is real unless we meet the criteria that no negative eigenvalue has odd multiplicity; see \citet{culver-1966-ExistenceMatrix}. \jackson{Do we care whether this is ever complex? We only use the logarithm to define powers, and we immediately exponentiate it...}
% \end{remark}

\begin{lemma} \label{lem:real_powers}
    Let $A$ be full-rank and diagonalizable as $WDW^{-1}$. Then $A^k = WD^kW^{-1}$ for $k \in \mathbb{R}$.
\end{lemma}

\begin{proof}
    We can extend the definition of matrix powers to non-integral values of $k$ by leveraging the equivalent form $A^k \coloneqq \exp(k \ln A)$, where $\exp$ and $\ln$ are the matrix exponential and logarithm respectively. Then
    \begin{align*}
        A^k &= \exp(k \ln A) \\
            &= \exp (k \ln W D W^{-1}) \\
            &= \exp \left(W k\ln(D) W^{-1}\right) \tag{\ref{lem:factor_log}} \\
            &= W \exp(k \ln D) W^{-1} \tag{\ref{lem:factor_exp}} \\
            &= W D^{k} W^{-1} \qedhere
    \end{align*}
\end{proof}

\begin{remark}
    Note that $A^k$ may not be uniquely defined for non-integral $k$, but can be consistently defined by arbitrary convention (similar to how $n^{1/2}, n \in \mathbb{Z}$ is only unique modulo a choice of positive or negative root, but we can arbitrarily decide to always choose the positive root).
\end{remark}



\begin{proposition}
    Let $A$ be full-rank and diagonalizable as $WDW^{-1}$. Then $\prod_i \exp(\delta_i A) = \exp(A)^{\sum_i \delta_i}$.
\end{proposition}

\begin{proof}
    \begin{align*}
        \prod_i \exp(\delta_i A) &= \prod_i W \exp(\delta_i D) W^{-1} \tag{\ref{lem:factor_exp}} \\
        &= W \left(\prod_i \exp(\delta_i D)\right) W^{-1} \\
        &= W (\prod_i \diag_j(e^{\delta_i d_{jj}})) W^{-1} \tag{$\star$} \\
        % &= W [e^{\delta_1 d_{jj}}] [e^{\delta_2 d_{jj}}] \cdots [e^{\delta_n d_{jj}}] W^{-1} \\
        &= W (\diag_j(e^{d_{jj}(\sum_i \delta_i)})) W^{-1} \\
        % &= W [e^{d_{jj}(\sum_i \delta_i)}] W^{-1} \\
        &= W \exp(D)^{\sum_i \delta_i} W^{-1} \\
        &= \exp(A)^{\sum_i \delta_i} \tag{\ref{lem:real_powers}}
    \end{align*}
    where $(\star)$ follows from the fact that the matrix exponential of a diagonal matrix coincides with the exponential applied to every element along the diagonal.
\end{proof}

Similarly, we can also extend the derivation of the S6 convolutional forms to consider full-rank, diagonalizable $A$.

\begin{lemma} \label{lem:diagonalizable-conv-form}
    Let $h_0 = \vec 0 \in \mathbb R^d$ and $h_i = \exp( \delta_i A ) h_{i-1} + B_i x_i \in \mathbb R^d$.
    Let $A$ be full-rank and diagonalizable as $WDW^{-1}$.
    Then for any $i \geq 0$,
    \begin{equation*}
        h_i = \sum_{j=1}^i B_i x_i W \exp \left( D \sum_{k=j+1}^i  \delta_k \right) W^{-1} .
    \end{equation*}
\end{lemma}


\begin{proof}
    \begin{align*}
        h_i
        &= \exp( \delta_i A ) h_{i-1} + B_i x_i  \\
        &= \sum_{j=1}^i B_i x_i \prod_{k=j+1}^i \exp( \delta_k A ) \\
        &= \sum_{j=1}^i B_i x_i \prod_{k=j+1}^i W \exp( \delta_k D ) W^{-1} \\
        &= \sum_{j=1}^i B_i x_i W \left(\prod_{k=j+1}^i \exp( \delta_k D ) \right) W^{-1} \\
        &= \sum_{j=1}^i B_i x_i W \exp \left( D \sum_{k=j+1}^i  \delta_k \right) W^{-1} . \qedhere
    \end{align*}
\end{proof}

==> old/suffix-indexing.tex <==
% \section{Comparing Transformers and SSMs}

\subsection{String Indexing Tasks}

Transformers and SSMs are both in $\TC^0$, but what can be said of their relative power? To investigate this, we define two variants of a string indexing task that are both naturally expressible by transformers but might challenge SSMs due to their bounded-size state.

\definecolor{babyblue}{rgb}{0.54, 0.81, 0.94}

\begin{figure}[]
    \centering
    \begin{tabular}{c}
        $\overbrace{\colorbox{pink}{$aaa \cdots a$}}^{\text{$i < n$ index tokens}} \overbrace{\colorbox{babyblue}{$bccbbc \cdots b$}}^{\text{$n$ data tokens}} \to \text{data\_tokens}[i]$ \\[1ex]
        $ \underbrace{\colorbox{babyblue}{$bccbbc \cdots b$}}_{\text{$n$ data tokens}} \underbrace{\colorbox{pink}{$aaa \cdots a$}}_{\text{$i < n$ index tokens}} \to \text{data\_tokens}[i]$
    \end{tabular}
    \caption{Pre- and post-indexing tasks for $V = \{b,c\}$.}
    % \caption{Pre- (above) and post-indexing (below) for $V = \{b,c\}$}
    \label{fig:string-indexing-illustration}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/copy_data.pdf}
    \caption{Minimum $d_\text{model}$ to attain $> 90\%$ validation accuracy on pre- and post-indexing tasks by sequence length $k$. \ashish{minor: change $k$ to $n$ in caption and figure}}
    \label{fig:string-indexing}
\end{figure}


We define the pre- and post-indexing tasks as classification problems. \cref{fig:string-indexing-illustration} provides an illustration. In the \textbf{pre-indexing task}, the input is a pair $\langle i, x \rangle$, where $x \in V^n$ is a string of length $n$ over a vocabulary $V$, $|V| = v$, and $0 \leq i < n$ is an index into this string. Operationally, the index $i$ is specified in unary notation, as $a^i$ where $a \not \in V$. The $v$-way classification task is to identify which element of $V$ is $x[i]$, the $i$-th entry of string $x$. We refer to each $a$ as an \emph{index token} and each $b$ and $c$ as a \emph{data token}. In the \textbf{post-indexing task}, the only difference is that the order of the inputs is flipped and specified as $\langle x, i \rangle$, i.e., the index $i$ comes \emph{after} the string $x$. This seemingly minor difference, as we will see, plays a crucial role.

% We define the prefix language $L_\textsf{pre} \coloneqq a^n \{bc\}^* \{bc\}$; we call $\{bc\}^*$ the data block. The final character $\{bc\}$ is equal to the $n$th character in the data block. The prefix $a^n$ indexes which character this is. The suffix language $L_\textsf{suf}$ is defined analogously, with the index $a^n$ appearing after $\{bc\}^*$ instead of before it. We generalize these languages by parameterizing the number of distinct characters $v$ which can appear in the data block and the maximum length $k$ of the data block.

% Transformers are capable of solving both variants of the task, since self-attention allows a model with at least two layers to first attend to the last position of the index and then to use that value as a key to identify the correct character from the data block. Whether the index comes before or after the data block does not impact the first layer's ability to attend to that position, so the two tasks are equally difficult for a Transformer. For state-space models, however, this is not the case.

% \will{Added discussion about similar experiments in literature}

Similar tasks have been used in the literature to benchmark the expressivity gap between transformers and SSMs. In particular, \citet{gu2023mamba} benchmarked Mamba on an \emph{induction head} task \citep{olsson2022incontext} very close to pre-indexing, but on nothing resembling post-indexing. \citet{fu2023hungry} evaluated H3 on both an induction head task and an \emph{associative recall} task very close to post-indexing, though H3 is not a true SSM architecture because contexts are not represented by a single state vector. In contrast, we wish to evaluate true SSMs on both of these tasks, expecting that the memory bottleneck of a single state vector will cause issues on the post-indexing task. The advantage of our post-indexing formulation compared to associative recall is that we capture both fundamental capabilities in a common string indexing framework, differentiated only by a single variable (the relative position of the data and index).

Both string-indexing tasks are naturally expressible by transformer-like models that, at the time of classification, can access a sequence of past hidden states. However, the two tasks differ in hardness for models that maintain only a single recurrent state. Intuitively, to solve the pre-indexing task in a recurrent fashion, one can first memorize $i$, then seek the $i$-th entry of $x$, memorize it, and use it at the end for classification. Solving the post-indexing task recurrently, however, is much harder. To see this, suppose the recurrent model, after reading input $x$, has created a hidden state $h_n$ of dimension $d$. In the case of log-precision SSMs, this state uses a total of $m = cd \log n$ bits. There are $2^n$ different possible values of $x$ but only $2^m = n^{cd}$ different possibilities for the hidden state $h_n$. Thus, as long as the hidden dimension $d$ is smaller than $n / (c \log n)$, multiple inputs $x$ must map to the same hidden state. The recurrent model therefore cannot distinguish between such strings, necessarily leading to classification errors on the indexing task. In general, by a simple counting argument, all input strings $x$ in a subset $S$ with $|S| \geq 2^{n-m} = 2^{n - cd \log n}$ must collapse to a single hidden state $h^*_n$, making the recurrent model fail on at least one index query (in fact, on roughly 
% $\O(\frac{n-m}{\log n})$
$\O((1 - \frac{m}{n}) / \log n)$ fraction of all
queries \ashish{added this, based on rough explanation on Slack. failing on `one index' is definitely very very conservative; got to fail on a lot more. but we also don't want to get into those details, too distracting}) for all but one string in $S$.
% \will{``not fully accurate on at least'' is weird.} \jackson{``must fail on''? if we consider perfect accuracy?} \will{cannot achieve perfect accuracy?} \will{The strange part is, IIUC, the model must not fail on all of these strings?}

% where the final character is the same as the $(2\cdot n)$th character; the prefix $a^n$ is called the index, since it indexes the identity of the final character $\{bc\}$ within the data block $\{bc\}^*$. The suffix language $L_\textsf{suf}$ is defined analogously, but with the index $a^n$ appearing after the $\{bc\}^*$ characters. Denote by $L_\textsf{pre}(v;k)$ the prefix (suffix) language with $v$ distinct characters that can appear in the data/final blocks, restricted to sequences whose data block is at most $k$ characters long.

% Define the prefix and suffix indexing tasks. The prefix version is the language of strings of the form $a^n \{bc\}^* \{bc\}$ such that the final character is the same as the $n$th character in the repetition of $b$'s and $c$'s.
% The suffix version is the same except that the idex $a^n$ is presented after the data $\{bc\}^*$.

% S4: No prefix or post-indexing
% S6: Can do prefix indexing
% Transformers: Can do both

\Cref{fig:string-indexing} compares transformer and S6 (Mamba) models of varying model dimensions on the pre- and post-indexing task (with $v=5$ distinct data characters) for successively longer sequence lengths. 

Both models can achieve perfect validation accuracy on the pre-indexing task with a fixed hidden size. On post-indexing, transformers achieve perfect performance with a fixed hidden size, but, for Mamba, the hidden dimension must increase for longer sequences lengths.
\will{complete once we have new figure}
% We note that even though Mamba does not learn post-indexing, it still does manage to attain better-than-chance accuracy; this is likely because models attempt to solve the task by memorizing as much of the data block sequence as they can in their state representation and then querying for the indexed character once it processes the end of the index tokens. To mitigate the models' ability to learn to memorize sequences, we consider the smallest model (as measured by the \texttt{d\_model} dimension) which can successfully solve the pre-index variant of the task and test to see if a model of that size can likewise solve the post-indexing variant. In practice, we compare 2-layer SSMs and Transformers with model dimensions of $8$. 

% \jackson{[...] Will, can you make this precise? My understanding of the hypothesis from our discussion on Monday was that an SSM could effectively learn to memorize the first $\ell$ tokens of the data block by compressing it into its state representation and then query that representation once it learns what the index is?} \will{Adding a note here about hashing construction from discussion. Idea: at each data entry, hash (token, position) and add it to a running sum vector. Then, at final position, hash ($a$, position) and ($b$, position), and check correlation with running sum vector. If there is any correlation, we know that is the right token}; 
